Designing Concise ConvNets with Columnar Stages

In the era of vision Transformers, the recent success of VanillaNet shows the huge potential of simple and concise convolutional neural networks (ConvNets). Where such models mainly focus on runtime, it is also crucial to simultaneously focus on other aspects, e.g., FLOPs, parameters, etc, to strengthen their utility further. To this end, we introduce a refreshing ConvNet macro design called Columnar Stage Network (CoSNet). CoSNet has a systematically developed simple and concise structure, smaller depth, low parameter count, low FLOPs, and attention-less operations, well suited for resource-constrained deployment. The key novelty of CoSNet is deploying parallel convolutions with fewer kernels fed by input replication, using columnar stacking of these convolutions, and minimizing the use of 1x1 convolution layers. Our comprehensive evaluations show that CoSNet rivals many renowned ConvNets and Transformer designs under resource-constrained scenarios. Code: https://github.com/ashishkumar822/CoSNet

==> images/cam_plot.tex <==


\begin{figure}[!h]

\centering

\FPeval{\imw}{12.0}
\FPeval{\imh}{12.0}


\vspace{-4.2ex}

\begin{tikzpicture}

\node (resnet) []{
\tikz{
%
%\node (outer) [draw=white!20!gray, rounded corners=0.2ex, minimum height =25ex, minimum width=43ex, xshift=15ex, yshift = -8ex]{};
%
\node (im1) [xshift=0ex]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/1500.png}};
\node (im3) [xshift=1*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/5000.png}};
\node (im5) [xshift=2*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/11000.png}};
\node (im5) [xshift=3*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/11500.png}};
\node (im5) [xshift=4*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/15500.png}};
\node (im5) [xshift=5*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/26500.png}};
\node (im5) [xshift=6*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/35500.png}};
%
\node (im1) [xshift=0ex, yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_resnet50/1500_heatmap.png}};
\node (im3) [xshift=1*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_resnet50/5000_heatmap.png}};
\node (im5) [xshift=2*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_resnet50/11000_heatmap.png}};
\node (im5) [xshift=3*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_resnet50/11500_heatmap.png}};
\node (im5) [xshift=4*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_resnet50/15500_heatmap.png}};
\node (im5) [xshift=5*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_resnet50/26500_heatmap.png}};
\node (im5) [xshift=6*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_resnet50/35500_heatmap.png}};
%
\node (im1) [xshift=0ex, yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/1500_heatmap.png}};
\node (im3) [xshift=1*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/5000_heatmap.png}};
\node (im5) [xshift=2*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/11000_heatmap.png}};
\node (im5) [xshift=3*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/11500_heatmap.png}};
\node (im5) [xshift=4*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/15500_heatmap.png}};
\node (im5) [xshift=5*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/26500_heatmap.png}};
\node (im5) [xshift=6*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/xcam_comnetb1/35500_heatmap.png}};
%
\node () [xshift=-7.0ex, yshift=0.0ex, rotate=90, scale = 1.0]{Image};
\node () [xshift=-7.0ex, yshift=-12.5ex, rotate=90, scale = 1.0]{ResNet-$50$};
\node () [xshift=-7.0ex, yshift=-24.5ex, rotate=90, scale = 1.0]{\OursNet{}-B$1$};
}
};

\end{tikzpicture}
%
\vspace{-4ex}
%
\caption{Axiom-GradCAM \cite{axiomcam} visualizations}
\label{fig:axiomcam}
%
%

\vspace{-1ex}
%
\end{figure}
%

%

\begin{figure}[!h]

\centering

\FPeval{\imw}{12.0}
\FPeval{\imh}{12.0}


\vspace{-4.2ex}

\begin{tikzpicture}

\node (resnet) []{
\tikz{
%
%\node (outer) [draw=white!20!gray, rounded corners=0.2ex, minimum height =25ex, minimum width=43ex, xshift=15ex, yshift = -8ex]{};
%
\node (im1) [xshift=0ex]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/3000.png}};
\node (im3) [xshift=1*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/4000.png}};
\node (im5) [xshift=2*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/6500.png}};
\node (im5) [xshift=3*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/9500.png}};
\node (im5) [xshift=4*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/11000.png}};
\node (im5) [xshift=5*(\imw ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/11500.png}};
%
\node (im1) [xshift=0ex, yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_resnet50/3000_heatmap.png}};
\node (im3) [xshift=1*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_resnet50/4000_heatmap.png}};
\node (im5) [xshift=2*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_resnet50/6500_heatmap.png}};
\node (im5) [xshift=3*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_resnet50/9500_heatmap.png}};
\node (im5) [xshift=4*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_resnet50/11000_heatmap.png}};
\node (im5) [xshift=5*(\imw ex+0.25ex), yshift=-1*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_resnet50/11500_heatmap.png}};
%
\node (im1) [xshift=0ex, yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/3000_heatmap.png}};
\node (im3) [xshift=1*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/4000_heatmap.png}};
\node (im5) [xshift=2*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/6500_heatmap.png}};
\node (im5) [xshift=3*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/9500_heatmap.png}};
\node (im5) [xshift=4*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/11000_heatmap.png}};
\node (im5) [xshift=5*(\imw ex+0.25ex), yshift=-2*(\imh ex+0.25ex)]{\includegraphics[width=\imw ex, height=\imh ex]{rebuttal_images/fullgrad_comnetb1/11500_heatmap.png}};
%
\node () [xshift=-7.0ex, yshift=0.0ex, rotate=90, scale = 1.0]{Image};
\node () [xshift=-7.0ex, yshift=-12.5ex, rotate=90, scale = 1.0]{ResNet-$50$};
\node () [xshift=-7.0ex, yshift=-24.5ex, rotate=90, scale = 1.0]{\OursNet{}-B$1$};
}
};

\end{tikzpicture}
%
\vspace{-2ex}
%
\caption{Full Gradient CAM \cite{fullgradcam} visualizations}
\label{fig:fullgradcam}
%
%

\vspace{-2ex}
%
\end{figure}
%



==> images/comnet_vs_inception.tex <==
\begin{figure}[!h]
\centering
%%

\subfloat[A stage of Inception \cite{googlenet}.]
{
\includegraphics[scale=0.2]{images/inception.pdf}
}
%
\hspace{6ex}
%
\subfloat[A stage of proposed CoMNet.]
{
\includegraphics[scale=0.40]{rebuttal_images/comnet_stage.png}
}




\caption{Difference between Inception \cite{googlenet} and CoMNet stage.}
%
%\vspace{-2.5ex}
%
\label{fig:inception_vs_comnet}
%
%
%
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

